Inclusive results for electron and photon scattering in the resonance region

We present a model for electron scattering off nuclei and photon absorption in the resonance energy region (W <= 2 GeV). The elementary gamma/gamma* N-vertex is described using in-medium kinematics and up-to-date form factors for QE-scattering, pion-production form-factors and resonance helicity amplitudes of the MAID analysis. We find good agreement with inclusive data on electron scattering off Oxygen. For photon absorption in Carbon we find a large impact of the momentum dependent mean-field acting on initial- and final-state baryons.

==> buu.tex <==
Boltzmann-Uehling-Uhlenbeck (BUU) transport models are based on the Boltzmann equation, which was modified  by Nordheim, Uehling and Uhlenbeck to incorporate quantum statistics. A brief description of the formalism is given below. For a detailed discussion concerning the physical input for pion-induced reactions we refer the reader to~\cite{Buss:2006vh,Buss:2006yk} and the references therein. 

\subsection{The BUU equation}\label{buuEQ}
The BUU equation actually consists of a series of coupled differential equations, which describe the time evolution of the \newla{single}-particle \newla{phase-space densities $f_a(\vec{r},\vec{p},t)$. The index $a=\pi,\omega,N,\Delta,\ldots$ denotes the different particle species in our model.} A large number of mesonic and baryonic states is actually included, but at the energies of interest for this study, the relevant ones are $\pi,N$ and the $\Delta(1232)$ resonance.

For a particle of species X, its time evolution is given by
\begin{eqnarray}
&&\frac{d f_X(\vec{r},\vec{p},t)}{d t}=\frac{\partial f_X(\vec{r},\vec{p},t)}{\partial t} +\frac{\partial H_X}{\partial \vec{p}}\frac{\partial f_X(\vec{r},\vec{p},t)}{\partial \vec{r}} \nonumber
\\  &&-\frac{\partial H_X}{\partial \vec{r}}\frac{\partial f_{X}(\vec{r},\vec{p},t)}{\partial \vec{p}}   %&
=I_{coll}\left(f_X,f_a,f_b,\ldots\right)
\label{BUUEquation}
\end{eqnarray}
with the one-body Hamilton function 
\begin{eqnarray}
%H_X(\vec{r},\vec{p})&=&\sqrt{\left(\vec{p}+\vec{A}_X(\vec{r},\vec{p})\right)^{2}+m_X^{2}+U_X(\vec{r},\vec{p})}\nonumber\\ && +A_X^{0}(\vec{r},\vec{p})
H_X(\vec{r},\vec{p})&=&\sqrt{\left(\vec{p}-\vec{A}_X(\vec{r},\vec{p})\right)^{2}+m_X^{2}+U_X(\vec{r},\vec{p})}\nonumber \\
&& +A_X^{0}(\vec{r},\vec{p}) \; .
\label{HamiltonFunc}
\end{eqnarray}
The scalar potential $U_X$ and the vector potential $A^\mu_X$ of species X may in principle depend upon the phase space densities of all other species. Hence, the differential equations are already coupled through the mean fields. In the limit of $I_{coll}=0$, eq.~(\ref{BUUEquation}) becomes the well-known Vlasov equation. The collision term $I_{coll}$ on the right-hand side of eq.~(\ref{BUUEquation}) incorporates explicitly all scattering processes among the particles. The  reaction probabilities used in this collision term are chosen to match the elementary collisions among the particles in vacuum. Therefore, we model these probabilities as a sum of dominant resonance terms and small background terms. The latter resonance terms are based on the partial wave analysis of Manley et al.~\cite{ManleySaleski}. The background terms are defined as differences between experimental data and resonance contributions. Note that background contributions are instantaneous in space-time, whereas the resonances propagate along their classical trajectories until they decay or interact with one or two nucleons in the medium. 

Concerning pion absorption, the most important mechanisms are a two step process in which $\pi N \to \Delta$ is followed by $\Delta N \to NN$ \new{or $\Delta N N \to NNN$}, and the one step background process $\pi N N \to N N$. 

\subsection{Medium effects}
\label{mediumEffects}
As medium modifications, we include Pauli-blocking and Fermi-motion of the nucleons and Coulomb forces. Furthermore, we account for the collisional broadening in the $\Delta$ resonance width. The hadronic potentials included are introduced as \cor{time-like} components of vector potentials in the local rest-frame~\cite{Teis:1996kx}. For our purposes the most important mean field potentials are those acting on the nucleon and the $\Delta$ resonance. The nucleon mean-field potential is parametrized by Welke et al.~\cite{Welke} as a sum of a Skyrme term depending only on density and a momentum-dependent contribution (for explicit details and parameters see~\cite{Teis:1996kx}). Phenomenology tells us that the $\Delta$ potential  has a depth of about $-30 \MeV$ at $\rho_{0}$\,\cite{ericsonWeise,Peters:1998mb}. Comparing to a momentum independent nucleon potential, which is approximately $-50 \MeV$ \cor{deep}, the $\Delta$ potential is, \cor{therefore,} taken to be
\begin{eqnarray*}
        A^0_{\Delta}(\vec{p},\vec{r})=\frac{2}{3}\ A^0_{\mathrm{nucleon}}(\vec{p},\vec{r}).
        \label{DeltaPotential}
\end{eqnarray*}
Here we \cor{assume} the same momentum dependence for the nucleon and the $\Delta$ potential. No potential for the pion was included in the calculations.

